Cache-Aided MIMO Communications: DoF Analysis and Transmitter Optimization

Cache-aided MIMO communications aims to jointly exploit both coded caching~(CC) and spatial multiplexing gains to enhance communication efficiency. In this paper, we analyze both the achievable degrees of freedom~(DoF) under linear processing constraint and the finite-SNR performance of a MIMO-CC system with CC gain \(t\), where a server with \(L\) transmit antennas communicates with \(K\) users, each equipped with \(G\) receive antennas. We first demonstrate that the enhanced DoF of \(\max_{\beta, \Omega} \Omega \times \beta\) is achievable with linear processing, where the number of users \(\Omega\) served in each transmission is fine-tuned to maximize DoF, and \(\beta \le \min\big(G, \nicefrac{L \binom{\Omega-1}{t}}{\big(1 + (\Omega - t - 1)\binom{\Omega-1}{t}}\big)\big)\) represents the number of parallel streams decoded by each user. Then, we propose a new class of MIMO-CC schemes using a novel scheduling mechanism leveraging maximal multicasting opportunities to maximize delivery rates at given SNR levels while still adhering to linear processing constraints. This new class of schemes is paired with an efficient linear multicast beamformer design, resulting in a more practical, high-performance solution for integrating CC in future MIMO systems.

==> Figs/DoF_Prop_SOTA.tex <==
TxAntenna		dofucTH1t2G16		dofmcTH3t2G16		dofwsat2G16		dofextMSt2G16		dofucTH1t2G8		dofmcTH3t2G8		dofwsat2G8		dofextMSt2G8		dofucTH1realbetat2G16		dofucTH1realbetat2G8		dofmimoG8	
1		3		3		3		3		3		3		3		3		3		3		1	
2		6		6		4		3		6		6		4		3		6		6		2	
3		9		9		5		3		9		9		5		3		9		9		3	
4		12		12		6		12		12		12		6		12		12		12		4	
5		15		15		7		12		15		15		7		12		15		15		5	
6		18		18		8		12		18		18		8		12		18		18		6	
7		21		21		9		12		21		21		9		12		21		21		7	
8		24		24		10		12		24		24		24		12		24		24		8	
9		27		27		11		12		24		24		24		12		27		27		9	
10		30		30		12		12		28		24		24		12		30		30		10	
11		33		33		13		12		32		24		24		12		33		32		11	
12		36		36		14		12		32		24		24		12		36		32		12	
13		39		39		15		30		32		30		24		30		39		32		13	
14		42		42		16		30		32		30		24		30		42		32.30769231		14	
15		45		45		17		30		32		30		24		30		45		34.61538462		15	
16		48		48		48		30		35		30		32		30		48		36.92307692		16	
17		48		48		48		30		35		30		32		30		51		39.23076923		17	
18		52		48		48		30		40		30		32		30		54		40		18	
19		56		48		48		30		40		36		32		30		57		40		19	
20		60		60		48		30		40		36		32		30		60		40		20	
21		60		60		48		30		40		36		32		30		63		40.64516129		21	
22		64		60		48		30		42		42		32		30		64		42.58064516		22	
23		64		60		48		30		42		42		32		30		64		44.51612903		23	
24		64		60		48		30		42		42		40		30		64		46.4516129		24	
25		64		60		48		30		48		48		40		30		64		48		25	
26		64		60		48		30		48		48		40		30		64		48		26	
27		64		60		48		30		48		48		40		30		64		48		27	
28		64		60		48		30		48		48		40		30		64.61538462		48.19672131		28	
29		65		60		48		30		49		48		40		30		66.92307692		49.91803279		29	
30		65		60		48		30		49		48		40		30		69.23076923		51.63934426		30	
31		70		60		48		60		49		48		40		30		71.53846154		53.36065574		31	
32		70		60		64		60		49		48		48		30		73.84615385		55.08196721		32	
33		75		75		64		60		56		48		48		30		76.15384615		56		33	
34		75		75		64		60		56		48		48		30		78.46153846		56		34	
35		80		75		64		60		56		48		48		30		80		56		35	
36		80		75		64		60		56		48		48		30		80		57.05660377		36	
37		80		75		64		60		56		54		48		30		80		58.64150943		37	
38		80		75		64		60		56		54		48		30		80		60.22641509		38	
39		80		75		64		60		56		54		48		30		80		61.81132075		39	
40		80		75		64		60		56		54		56		30		80		63.39622642		40	
41		80		78		64		60		64		54		56		30		80		64		41	
42		80		78		64		60		64		54		56		30		81.29032258		64		42	
43		80		78		64		60		64		63		56		30		83.22580645		64.1183432		43	
44		84		84		64		60		64		63		56		30		85.16129032		65.60946746		44	
45		84		84		64		60		64		63		56		30		87.09677419		67.10059172		45	
46		84		84		64		60		64		63		56		30		89.03225806		68.59171598		46	
47		90		90		64		60		64		63		56		30		90.96774194		70.08284024		47	
48		90		90		80		60		64		63		64		30		92.90322581		71.5739645		48	
49		90		90		80		60		72		72		64		30		94.83870968		72		49	
50		96		96		80		60		72		72		64		30		96		72		50	


==> Figs/DoF_Scalability1.tex <==
TxAntenna	dofG8propt1	dofG16propt1	dofG8propt3		dofG16propt3		dofGmimo
0	0	0	0		0		0
8	16	16	32		32		8
12	24	24	40		48		12
16	24	32	42		64		16
20	32	39	48		80		20
24	35	48	49		80		24
28	0	0	0		0		0


==> Figs/DoF_prop_behav.tex <==
Omega	dofG4	dofG8
0	0	0
2	8	16
3	12	24
4	16	24
5	20	20
6	18	18
7	21	21
8	16	16
9	18	18
10	10	10
11	11	11
12	12	12
13	13	13
14	14	14
15	15	15
16	16	16
17	17	17
18	0	0


==> Figs/Symmetric_rate_Prop_SOTA_Comparison.tex <==
SNR		L10G5t1COVOmega4beta4	L10G5t1MCOmega4beta4	L10G5t1MSOmega4beta3		L10G5t1UCmega4beta4		L11G31COVOmega5beta3			L11G31MCOmega7beta2			L11G31MSOmega4beta3			L11G31UCOmega5beta3			L7G21COVOmega5beta2			L7G21MCOmega8beta1			L7G2t1MCOmega6beta1			L7G2t1MSOmega3beta2			L7G2t1UCOmega5beta2				L10G5t1MCOmega5beta2			L10G5t1MCOmega6beta2			L10G5t1MCOmega10beta1			L10G5t1MCOmega2beta5			L7G2t1MCOmega4beta2			L7G2t0MIMOOmega7beta1				L11G3t0MIMOOmega11beta1				L7G2t1UCOmega8beta1			L11G3t1UCOmega12beta1				L7G5t0MIMOOmega7beta1				L7G5t2MCOmega5beta3			L7G5t2WSAUCOmega3beta5				L7G5t2WSAMCOmega3beta5			L7G5t2MSMCOmega4beta3			L11G8t2WSAUCOmega3beta8			L7G5t2UCOmega4beta5			L11G8t2MSOmega4beta3			L11G8t2MIMOOmega11beta1				L11G8t2UCOmega4beta8			L11G8t2MCOmega4beta6			L11G8t2UCOmega4beta6			L10G5t1MCOmega3beta4				L11G8t2MIMOOmega11beta1LC				L7G5t0MIMOOmega7beta1LC				L11G3t0MIMOOmega11beta1LC				L11G8t2UCOmega6beta3			L11G8t2UCOmega13beta1			L11G8t2MCOmega6beta3	
																																																																																																																																
0		17.66712752	16.37314284	16.5442815		12.24669571			15.11851717			14.4341494			13.09541218			11.05797837			8.849605698			8.828336777			8.567928323			7.226145442			6.687930866			17.17664902				17.72465868			17.97899133			12.86552765			7.366566742		6.180652419				10.88640011				6.802085421				11.76614853				9.490177567				18.73063237			11.31121732				16.85804911			17.90543759			17.18814349			11.6830728			28.2753526			16.5215342				18.27631654			29.44064021			18.27722011			15.22032145				18.35726022				10.54464174				11.45936854				19.17536716			18.87904057			32.11392584
5		32.30459832	29.44774627	30.38559099		23.26943779			27.53121353			26.32289686			24.17672401			20.57252238			16.61451555			16.53916752			15.65958557			13.74475402			12.63199606			30.21205956				31.96833357			31.19781693			22.58104006			13.89660494		11.6771951				20.41071468				12.76949045				21.69389213				17.52512117				34.82817927			21.62508052				29.51467053			32.92883944			33.50876385			22.68938359			46.81458065			29.89518291				35.82610503			53.61015278			35.83522691			27.67575114				33.2168699				19.47235686				21.48496282				36.77953012			34.24712288			56.54234607
10		51.8064144	46.71708257	47.94032533		38.9080525			43.59428436			42.25455348			38.89946343			33.90680269			26.69690803			26.59263991			24.59581774			22.32270614			20.56371635			45.83332422				49.73810117			46.93262199			34.84423649			22.81566742		19.74614438				34.03270907				21.14861873				35.2265362				27.65226561				56.40677956			37.0392688				46.56138912			51.9611147			58.11455554			39.00472592			67.66972678			46.1935403				62.01538674			87.31333665			62.22809985			44.45741235				51.32615589				30.72473957				35.82390428				62.09721269			54.00345224			86.08933471
15		75.00501331	68.48712869	67.58595465		58.31860061			62.02781049			61.42968567			56.48607385			49.68579347			38.56522976			38.45245389			34.46075188			32.02382119			29.77066668			62.64837947				69.43966742			63.74971977			48.38072572			33.76702252		29.80990418				50.37516475				31.45640426				51.25659801				38.75481115				81.4402272			57.47133916				65.32765466			72.96229346			90.70505057			59.70955086			89.40139827			63.7883347				96.28140625			127.0882656			96.58894529			63.76226294				70.87592744				43.06090128				53.02648921				91.79956459			76.22902964			117.8248297
20		100.2652701	93.35443275	88.08834975		78.82818777			82.66205292			82.27848761			75.95938346			66.74049899			52.08472915			52.03367286			44.73469201			42.2111423			39.3393401			79.90580244				90.09269453			81.08501647			62.5383867			46.10510769		40.86818513				67.85524366				43.4384501				69.43991014				50.208174				107.9471028			81.92514696				86.12892287			94.40887582			129.5831243			85.21748772			111.4124173			81.8120788				136.6759648			169.7135032			135.6574659			84.14221337				90.90230978				55.78686				71.42657227				123.7115126			99.58498822			150.7168216
25		127.2217077	119.9106016	108.9706152		100.7417822			106.1825871			106.0243338			96.33266705			84.53394352			66.77467422			65.32493464			55.15077048			52.58669514			50.06243522			97.18308537				110.9909422			98.3845738			76.44166608			59.26297992		52.30581359				85.90430339				56.53879987				89.22001548				61.77850248				135.3608179			108.4729419				104.1297563			116.677628			171.9130151			111.1718067			133.4971101			100.0049993				177.3442227			213.4521549			177.1563615			104.9283977				111.1166659				68.64278053				90.42558252				156.4810568			123.353208			183.626963
30		154.5364588	147.1912872	129.7591932		121.9154991			131.3585204			129.2657274			117.0804475			102.2809144			82.41259322			78.92819008			65.61510425			63.03243779			61.40578938			114.5177536				131.5184061			115.8151792			90.33175006			72.85914286		63.87129478				104.0944478				69.57516387				109.8627456				73.37267727				162.9361318			135.7846388				128.005555			138.8367876			215.5627451			139.3994987			155.4729654			118.2805777				220.6686294			257.5316089			222.0682732			125.7839278				131.4228641				81.52519697				109.5731029				189.564432			147.4257912			216.7836738

